In-Context Learning for Few-Shot Dialogue State Tracking

Collecting and annotating task-oriented dialogues is time-consuming and costly; thus, zero and few shot learning could greatly benefit dialogue state tracking (DST). In this work, we propose an in-context learning (ICL) framework for zero-shot and few-shot learning DST, where a large pre-trained language model (LM) takes a test instance and a few exemplars as input, and directly decodes the dialogue state without any parameter updates. To better leverage a tabular domain description in the LM prompt, we reformulate DST into a text-to-SQL problem. We also propose a novel approach to retrieve annotated dialogues as exemplars. Empirical results on MultiWOZ show that our method IC-DST substantially outperforms previous fine-tuned state-of-the-art models in few-shot settings. In addition, we test IC-DST in zero-shot settings, in which the model only takes a fixed task instruction as input, finding that it outperforms previous zero-shot methods by a large margin.

==> EMNLP 2022/sections/acknowledgements.tex <==
%\section*{Acknowledgments}
%We thank Ruiqi Zhong for generating test suite databases for our evaluation.
%%thank tianbao and chen too

==> EMNLP 2022/sections/analysis.tex <==
\section{Analysis}
\label{analysis}
\vspace{-2mm}

To better understand the effectiveness of our proposed methods, we provide detailed analysis in this section.
All ablation experiments are conducted on 100 random MultiWOZ 2.4 development set dialogues in the 5\% few-shot setting.
% \tao{consider to re-organize this section as 
% 1) effect of dialogue context representation (split Table~\label{analysis_prompting} into two tables.);
% 2) effect of DST as Text-to-SQL;
% 3) effect of dialogue retriever (finetuning vs. no finetuning; \# of in-context examples...);
% 4) effect of predicting state changes;
% 5) flexibility and scalability of IC-DST: zero-shot cross-domain;
% 6) Performance of un-trained system?;
% 7) qualitative error analysis.}

\input{tables/prompting}
%\paragraph{Comparison of prompting methods}
\paragraph{Representation of dialogue context}
\label{analysis_prompting}
Table~\ref{prompting_method} compares approaches to representing dialogue context in the examples in the prompt, with different retriever fine-tuning objectives. 
%%MO: The figure does not illustrate single turn, so I commented this sentence out
%These approaches are illustrated in Figure~\ref{fig:representation}.
For each setting, we train a retriever with the given dialogue context representation and retrieval objective for a fair comparison.
We experiment with representing the dialogue history by:
%%MO: the table description is self-explanatory and doesn't need the bolded stuff here
\textbf{(1)} 
%\textbf{full context}: 
concatenating the whole dialogue history,  
\textbf{(2)} 
%\textbf{single turn}: 
only the latest turn (one system utterance and one user utterance), and \textbf{(3)} 
%\textbf{prev. state + single turn}: 
the previous dialogue states and the latest turn.
For both of the retrieval objectives, representing the dialogue context by the previous dialogue state and the current turn gives the best performance. 
%\mari{If you have to truncate examples when using the full context, mention that. Codex isn't "discovering similarity" -- the retriever has that role.  I think that the possible explanations could be the truncation and/or the fact that the previous state is more relevant than the full context for predicting the next state.  This is especially going to be true after a topic shift.}
% One possible explanation is that Codex is better at discovering similarity between shorter texts, rather than long dialogues. Also, the result indicates that dialogue state can be viewed as a summary of the previous dialogue history. 
There are multiple possible explanations.
First, the previous state is more relevant than the full context for predicting the next-turn dialogue state, especially after a topic shift.
Second, full dialogue contexts are too long. To fit in the length limit of Codex, we sometimes need to truncate examples when using full context, which lowers the system performance, as evidenced by the fact that a single turn outperforms the full context but not the state-based representation.
%In addition, adding the previous dialogue state is better than using the single turn alone, showing that information from previous turns is helpful for dialogue understanding.


\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{fig/JGA_of_each_turn.pdf}
    \caption{JGA of each turn.  
    % \nascomment{can you increase font size in the figure's legend?  also remove title inside the graphic since it's redundant with the caption}
    The blue line is the JGA of state changes predicted by the system on Table~\ref{prompting_method} row 5 (our \NAME setting).
    The red line is the JGA of dialogue states produced by accumulating predicted state changes.
    The yellow line is the JGA  of dialogue states predicted by the system on Table~\ref{prompting_method} row 2.}
    \label{fig:turn_accuracy}
    \vspace{-4mm}
\end{figure}

\paragraph{Dialogue states vs.\ state changes}

%In Table~\ref{prompting_method}, 
We also explore the benefit of using state change vs.\ full dialogue state labels ($c_t$ vs.\ $y_t$).
%different example labels:
%\textbf{(1)} \textbf{dialogue states}: the aggregated dialogue state $y_t$ of the current turn, 
%and \textbf{(2)} \textbf{state changes}: only the state changes $c_t$ of the current turn. 
Note that example labels also act as the basis for the similarity objective in training the retriever.
%Note that our retriever's goal is to fetch samples with similar labels as the test instance. Thus, example labels also act as the retrieval objective.
%
Table~\ref{prompting_method} shows that using state changes gives substantial improvement.
%One possible explanation 
A likely reason is that state changes contain fewer slots compared with dialogue states, making for an easier prediction task for the LM.
Also, there are many more example turns with the same state changes, compared with examples with the same dialogue states,
making it
%. So, it is 
easier for the retriever to fetch good examples 
%with the same state changes, especially 
in few-shot scenario. 
%The better exemplar coverage leads to better model performance.

We further compare these two kinds of example labels by investigating the JGA on each turn, illustrated in Figure~\ref{fig:turn_accuracy}. 
Because states have increasing numbers of slots with more turns, JGA (red and yellow lines) of the full state decreases for later turns. However, all turns have a relatively small number of state changes, so the state change JGA (blue line) remains high throughout the dialogue.  As a result, the JGA of the full state benefits from using predicted state change updates (red line, Table~\ref{prompting_method} row 5) as compared to predicting the full state (yellow line, Table~\ref{prompting_method} row 2).
%The blue line and red line are from our \NAME model (Table~\ref{prompting_method} row 5).
%The blue line is the JGA of the predicted state change on each turn, and the red line is the JGA of dialogue states, produced by accumulating the state changes.
%The yellow line is the JGA of dialogue states from the system that directly outputs the full dialogue state during inference (Table~\ref{prompting_method} row 2). 
%It directly outputs the dialogue states during inference.

% The experiment is Codex trained with 5\% training data evaluated on MultiWOZ 2.4 dev set. 
%The blue line shows that the state change JGA is consistent across each turn, indicating that LM has high accuracy in predicting state changes.
%The red line shows that dialogue state JGA experiences a drop for each turn. The reason is that the mistakes of previous turn prediction cannot be fixed in the later turns.
%The yellow line experiences a steeper drop in the later turns, compared with the red line.
%It shows that using state changes is better than using dialogue states for both retriever training and in-context learning, especially for long dialogues.
% \mocomment{If time, add a curve for the case where you predict dialog state F1 in training the retriever. Alternatively, you could include a line in table 4 for this case.}

\input{tables/retrievers}


\paragraph{Performance dependence on the retriever}
\label{anaysis_retriever}
Table~\ref{retriever} compares Codex's performance when using different retrievers.
%\mari{You need to explain what F1 is computed over in the figure caption and/or the discussion. Is it state changes or the full state? Is it for the best example (e.g. for copy) and/or the union of state changes?}
$F_1$ is computed over the predicted and gold full dialogue states.
The ``copy'' baseline makes a prediction by copying the label of the nearest example retrieved by the corresponding retriever in the selection pool.
This baseline gives a direct measure of the quality of the retrieved examples.
First, the result shows that Codex's performance is highly dependent on the quality of the retrievers and their retrieved examples. 
We can also see that $F_1$ of ``copy'' baseline  correlates  with the end task performance (JGA), which supports the use of state-change $F_1$ as a learning objective for 
%the effectiveness of 
our similarity measure. 
%defined in 
%(Section~\ref{approach_retriever}). 
Our finetuned SBERT retriever obtains substantial improvements over the unsupervised one. 
The oracle retriever fetches the examples that have the highest state change $F_1$,  assuming prior knowledge of test instance gold dialogue states. It shows the upper bound of the retriever performance in this few-shot setting. Note that the state-of-the-art full-shot performance on MultiWOZ 2.4 is 73.62\%~\cite{ye2021slot}. The oracle experiment shows that 
%given a better retriever, our 
the few-shot ICL may match or outperform the state-of-the-art full-shot model
with further retriever improvements.
%, using only 5\% of data.


%\paragraph{The LM is \emph{not} simply copying the example labels}
Table~\ref{retriever} also shows that the LM is \emph{not} simply copying the example labels. For both evaluation metrics and all the retrievers, the ``copy'' baseline performance is much lower than \NAME, indicating that the inference language model is generalizing over the examples, rather than copying the closest example labels.
%%MO: This was already said in the Table 1 discussion and seems out of place here
%Also, the result in Table~\ref{mw2.1results} indicates that bigger model (Codex) tends to have stronger generalization ability over the smaller models (GPT-Neo 2.7B and CodeGen 2.7B).


% \paragraph{Performance of un-trained system}
% %Table ~\ref{unsupervised} 
% Figure ~\ref{fig:flexibility} shows the performance of \NAME with unsupervised SBERT retriever on each domain of MultiWOZ 2.4 development set. The system do not need any training. The model gets decent performance with only 1\% training data as selection pool, and the performance is better when more samples is added to the selection pool. The results show the flexibility and scalability of our \NAME in practice. When new slots are added to the schema, or samples from an unseen domain are added, users simply need to update the SQL tables in the prompt and add the new samples to the selection pool. The model is able to perform well without any re-training. 

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=\linewidth]{fig/DB_untrained.pdf}
%     \caption{Single-domain JGA on MultiWOZ 2.4 dev set of \NAME with unsupervised SBERT retriever, given 1\% and 100\% training data as selection pool. The system does not need any training.}
%     \label{fig:flexibility}
% \end{figure}

%%MO: moved to appendix
%\input{tables/flexibility}

\input{tables/formulation}
%\paragraph{Comparison of different task formulation}
%\input{tables/errors}
\paragraph{Effect of DST as Text-to-SQL}
Table~\ref{formulation} shows the performance of our ICL framework given different input-output formats. 
We follow SimpleTOD~\cite{hosseini2020simple} as the traditional format to formulate the input-output.
More specifically, the exemplar labels and the generation target are slot-value pairs.
% \tao{Yushi to add more details}
Also, we rewrite the dialogue schema in the same format in the prompt to replace the SQL tables.
The prompt in the setting is shown in Appendix~\ref{appendix:traditional}.
By reformulating DST as a text-to-SQL task, and leveraging large language models pretrained with code, ICL can make better use of the structured knowledge associated with the task schema. 
%as mentioned in Section~\ref{sec:task-framing}, large language models pre-trained with code can be better exploited.
As shown in Table~\ref{formulation}, GPT-Neo, CodeGEN, and Codex all perform better with text-to-SQL format.
Note that the performance of GPT-Neo with the traditional format is much worse than with the text-to-SQL format, possibly
%One reason could be its limited input-output generalization ability, 
due to its much smaller model size compared to Codex. It is easier for GPT-Neo to work with SQL, rather than learning a slot value pair format. 



%\paragraph{Comparison of different task formulation}
% \paragraph{What is the best generation target?}
% Table ~\ref{formulation} shows the performance of our in-context learning framework given different generation target formats. 
% We follow the format in SimpleTOD~\cite{hosseini2020simple} as the traditional format. 
% By reformulating DST as a text-to-SQL task, large language models pre-trained with code can be better exploited. 
% Both Codex and GPT-Neo perform better with text-to-SQL format.
% % \tao{somehow similar to the first parap, maybe renaming first parap}
% \input{tables/formulation}



%%MO: I think the boldface in the text is confusing with the paragraph headers, so I changed it to italics

%%MO: I move the table to the appendix, together with the explanation of specific examples

\paragraph{Error analysis}

\input{tables/errors}


In examining a subset of \NAME errors, we identified three common types, 
as shown in Table~\ref{tab:common error}.
%(see Table~\ref{tab:common error}, Appendix~\ref{appendix:errors}, for examples).
%shows some common error types of \NAME. 
The first type of error is caused by a \textit{noisy training example}, such as a missing slot. 
ICL is sensitive to noisy training data because the inference LM only sees a few examples in the prompt during prediction. 
%The mistakes in these examples will lead to mistakes in prediction.
%
%The second type of error is \textbf{missing named entities}.
%Because the inference LM has not been trained with task-specific data, it cannot recognize the named entities in the dataset. 
%In this example, the LM fails to recognize `city centre north bed and breakfast' is a hotel name. 
%
%One possible fix is to provide  hint of named entities in the dialogue via an auxiliary system.
The second type of error is \textit{retrieval limitations}. 
%Different from the first case, there is no annotation error in the examples. However,
In this case, the retrieved samples are not good exemplars, because they lack some slots that should be predicted in the test instance. This could be due to sparse annotated data (which impacts all few-shot learning methods) or a retriever error.
%In this example, the inference LM is mimicing the example, only predicting slot `attraction-name' and missing the slot `hotel-pricerange'. 
%
The third type of error is \textit{failure to generalize from examples}, which happens when the model fails to learn from examples. 
%In this example, the in-context example contains the notion of slot value `don't care'. However, the LM fails to generalize this notion and misses the slot value pair `hotel-area: don't care'.
%%MO: I don't think that you can make this claim unless there are better examples that you could have retrieved
%We can reduce this type of error by improving the retriever.








==> EMNLP 2022/sections/approach2.tex <==
\section{DST System Design}

\subsection{DST Task Framing}
\label{sec:task-framing}
\paragraph{Notation}
A task-oriented dialogue consists of a sequence of utterances alternating between the user and the system, $A_1, U_1, ..., A_T, U_T$, where $A$ and $U$ represent the system and user utterances, respectively.
The task of DST is to predict the dialogue state $y_t$ at each turn $t$,\footnote{For brevity, ``turn'' is used to mean a pair of system and user turns $(A_t, U_t)$, 
associated with state update intervals.}
%since the dialogue state is only updated after a user turn.} 
given the dialogue context $C_t = [A_1, U_1, \cdots, A_t, U_t]$, where
$y_t$ is a set of slot-value pairs: 
%\nascomment{please check my fix from y to v below}
%\begin{align*}
%    y_t = \{(s_1, v_1)_t, (s_2, v_2)_t, \cdots, (s_{n_t}, v_{n_t})_t\}
%\end{align*}
%\begin{align*}
%    y_t = \{(s_{t,1}, v_{t,1}), (s_{t,2}, v_{t,2}), \cdots, (s_{t,n_t}, v_{t,n_t})\}
%\end{align*}
%\begin{align*}
%    y_t = \{(s_{t,i}, v_{t,i}); i=1,\ldots , n_t\}
%\end{align*}
\begin{align*}
    y_t = \{(s_i^t, v_i^t); i=1,\ldots , n_t\} .
\end{align*}
%\mari{There needs to be a "t" on both sides of the equation.  I'm not sure what is the best way to do that.}
The set of possible slots ${s_i}$ is given in a pre-defined schema. 
The schema can contain multiple domains,
where a ``domain'' corresponds to a backend capability such as hotel or restaurant booking. Each domain is associated with a set of slots;
for example, the `hotel' domain has slots `hotel-name', `hotel-price\_range,' `hotel-area', etc. 
Each observed slot is associated with a value, which may have pre-defined categories (e.g., `hotel-price\_range' may be `cheap,' `moderate,' or `expensive') or open (e.g.\ `hotel-name').
We focus on a multi-domain scenario in this work, in which dialogue states may contain slots from multiple domains.  

One popular way to generate the dialogue states for the current turn is finetuning auto-regressive language models \cite{hosseini2020simple,peng2020soloist}. For each turn, the model takes the dialogue context $C_t$
%$C_t = [A_1, U_1, \cdots, A_t, U_t]$ 
as input, and generates a sequence of slot-value pairs $(s_i, v_i)$ sequentially.
Equivalently, one can generate a sequence of slot-value pair dialogue state changes.

\paragraph{Dialogue states vs.\ state changes}
\label{approach_statechange}

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=\linewidth]{fig/state-changes.pdf}
%     \caption{Illustration of the DST task, which involves tracking the slot values associated with a user request up to the current turn (dialogue state). Equivalently, we predict state change labels, shown here in slot-value and SQL format.}
%     \label{fig:state-changes}
% \end{figure}

Dialogues can be lengthy and complex, resulting in dialogue states that can include several slots and values, which means that coverage of the possible states is sparse for few-shot learning. However, the dialogue state change from one turn to the next typically involves a small number of slots. For that reason, we use state \emph{changes} at each turn as a label for prediction.
The concept of state changes is illustrated in Figure~\ref{fig:system}.
Possible state changes include slot addition, slot deletion, and slot value change.  
For example, in the current test turn of Figure~\ref{fig:system}, the user asks for Catalan food in turn $t-1$, and changes it to French food in turn $t$.
The state change updates the dialogue state by replacing `Catalan' with `French'. 
Specifically, given the previous turn dialogue state $y_{t-1}$ and the predicted current turn state changes $c_t$, we update the dialogue state by first copying $y_{t-1}$ to $y_t$, and then executing add, delete and change operations according to each slot-value pair $(s_i,v_i)$ in $c_t$.
Our analysis in Section~\ref{analysis_prompting} shows that using state changes leads to substantial improvements.

%Given the previous turn dialogue state $y_{t-1}$ and the predicted current turn state changes $c_t$, we update $y_{t-1}$ by $c_t$ to predict the dialogue state at current turn $y_t$.
%We first copy $y_{t-1}$ to $y_t$. 
%For each slot-value pair $(s_i,v_i)$ in $c_t$, if $v_i=[\mathit{DELETE}]$, then we delete $s_i$ from $y_t$.
%If $s_i$ is not in $y_{t-1}$, then we add $(s_i,v_i)$ to $y_t$.
%Otherwise, $s_i$ is in $y_{t-1}$, and we change the value of $s_i$ to $v_i$ in $y_t$.

\paragraph{DST as Text-to-SQL}
Here we propose a new representation for dialogue states: SQL. This is inspired by the fact that dialogue states are used to determine how to query backend databases for the information users need. Our representation follows three rules: (1) each domain 
is defined as a table and each slot is defined as a column; (2) all the slots and values are in the WHERE clause; and (3) for turns with multiple domains, we rename each domain to $d_1, ..., d_m$. 
Using the SQL state representation with a generative LM, DST becomes a Text-to-SQL problem. This approach is facilitated by language models  pretrained with code (Codex and GPT-Neo) as SQL is closer to the code used for pre-training.

\paragraph{Dialogue context representation}
\label{approach_history}

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{fig/dialogue_history_plot.png}
    \caption{
    Illustration of the dialogue context representation: 
    the full dialogue context $C_{t-1}$ before the current turn is replaced by the associated dialogue state $y_{t-1}$. 
%    Instead of using the full dialogue context $C_{t-1}$ before the current turn, we represent the dialog history by dialogue state of the previous turn $y_{t-1}$.
    }
    \label{fig:representation}
    \vspace{-3mm}
\end{figure}

Previous work generally represents dialogue context by concatenating all the system and user utterances $A_1, U_1, \cdots, A_t, U_t$~\cite{lee2021dialogue, lin2021leveraging, peng2020soloist}. 
However, real world dialogues can be lengthy, and there is a length limit for current large language models (2048 tokens for GPT-3, 4096 tokens for Codex). 
It is not practical to represent full dialogue context for multiple exemplars in the prompt. 
%An alternative approach 
A simple solution is to just include the $N$ recent turns in the dialogue history~\cite{lei-etal-2018-sequicity, budzianowski2019hello, wu-etal-2021-dialki}. 
We adopt a new approach that takes advantage of the fact that the dialogue state is a summary of the dialogue history, as shown in Figure~\ref{fig:representation}.
Specifically, 
%we only use the agent-user utterances in the last turn, i.e.\ 
we represent dialogue context by $[y_{t-1}, A_t, U_t]$, in which $y_{t-1}$ is the accumulated dialogue state after user turn $t-1$.

\subsection{In-Context Learning}

% \begin{figure}
%   \includegraphics[width=0.48\textwidth]{fig/system-single-col.pdf}
%   \caption{
%   The \NAME approach in the few-shot setting.
%   A retriever takes the test turn as input and retrieves a few most similar turns from the labeled dialogues as demonstration examples.
%   The task schema, examples, and the current dialogue turn are concatenated together as the prompt to a pretrained LM (e.g., GPT3 or Codex) to produce the current turn dialogue state changes as a SQL query. 
% %   \mari{You need to change the figure: "Dialog ontology" should be "Task schema" or "Domain schema". The ontology is related to the task not the dialogue.}
%   }
%   \vspace{-2mm}
%   \label{fig:system}
% \end{figure}

\begin{figure}
  \includegraphics[width=0.48\textwidth]{fig/prompt.pdf}
  \caption{
%  Details of the prompt we use.
  The prompt contains the task schema, in-context examples, and the current test dialogue turn.
%  We use the dialogue context representation discussed in Section~\ref{approach_history} and represent the state change labels as SQL queries.
%\yushi{may skip this image to save some space?}
%%MO: I prefer to keep it if we can
  }
  \vspace{-3mm}
  \label{fig:prompt}
\end{figure}


\textit{In-context learning} is an alternative to finetuning that keeps pretrained language model parameters fixed~\cite{brown-gpt3}.
The language model takes a prompt $P$ that contains task descriptions, in-context examples, and the test instance as input, and predicts the label by capturing the patterns in the context.
%While finetuning the whole model has been a successful paradigm, 
ICL has two advantages over finetuning.
First, it avoids the need for repeated finetuning when the  schema is updated or new examples are added. 
This is particularly important for large models like GPT-3, since finetuning at this scale is extremely expensive. 
Second, by simply adding/removing training examples, in-context learning enables us to quickly manipulate the model's predictions and correct mistakes without re-training.

An overview of our \NAME system is shown in Figure~\ref{fig:system} for the few-shot setting.
The details of our prompt are shown in Figure~\ref{fig:prompt}.
The task description is the schema associated with the task ontology, and a retriever is used to select labeled example turns from the training data.
In the zero-shot setting, there is no retriever.




\paragraph{Schema prompting}
We use an SQL table for each domain to represent the dialogue schema in the prompt. Each table includes a row of slot names followed by three rows of example values associated with each slot, as illustrated in Figure~\ref{fig:schema}.  
%\mari{Can you add a sentence explaining ways in which the table is incomplete, e.g. not all possible slot values are listed?}
Slots like ``restaurant-name'' or "restaurant-book time" typically have many possible values. Thus, for these slots, we only list a few example values.
%cannot list all possible slot values in the prompt. 
In our experiments, we create SQL tables for all domains and concatenate them to be part of our input. 

\begin{figure}[t]
    \centering
    \includegraphics[width=0.9\linewidth]{fig/schema.png}
    \caption{The SQL table for the taxi domain schema. %There is one such SQL table for each domain in the prompt. 
    We follow the table prompt from \citet{Rajkumar2022EvaluatingTT}.
    %for Codex.
    }
    \label{fig:schema}
    \vspace{-3mm}
\end{figure}

\paragraph{In-context examples}
In the few-shot scenario,
a retriever takes the dialogue context as input (either $[C_{t-1}, A_t, U_t]$ or $[y_{t-1}, A_t, U_t]$) and retrieves similar example contexts from the labeled training set.
Advantages of using the dialogue state $y_{t-1}$ rather than the full history $C_{t-1}$ are that it is shorter (allowing for more examples) and it leads to a more effective retrieval similarity score.
In the zero-shot scenario, following previous work on zero-shot learning~\cite{wang2022benchmarking}, the in-context example is a formatting example turn.
We call this setting ``zero shot'' because the prompt is fixed by the system developer and does not use any labeled data. 
%
Prompt examples for the few-shot and zero-shot settings are given in Appendices~\ref{appendix:few shot} and \ref{appendix:zero shot}, respectively.

\subsection{Dialogue Retriever}
\label{approach_retriever}
In few-shot settings, successful prediction of in-context learning relies on the quality of the context examples. 
Usually this is accomplished by semantic retrieval using the testing input as the query. 
Previous studies have explored methods for building sentence-level retrievers~\cite{poesia2022synchromesh,rubin2021learning}. 
Our work goes beyond sentences 
%and studies how to retrieve dialogues.
to retrieving dialogue histories (contexts).

We want to retrieve example dialogue contexts that are relevant for the predicted state change of a test sample. 
Formally, suppose $X=\{(e_i,c_i)\}$ is a dataset of dialogue context $e_i$ and corresponding state change $c_i$ pairs. 
Each labeled turn in a dialogue is a candidate. 
Given a test dialogue context $x$, our goal is to retrieve $k$ examples $\{(e_1, c_1), (e_2, c_2), \cdots, (e_k, c_k)\}$ such that $c_1, c_2, \cdots, c_k$ should be similar to the state changes associated with $x$. 

\paragraph{Unsupervised retriever}
One approach is to use a pretrained embedding model with a cosine similarity score as the retriever. This approach does not need any DST data.  
Let $M$ be an embedding model.
For each test example $x$, 
we retrieve the $k$ training examples such that $e_i, e_2, \cdots, e_k$ are the nearest neighbors of $x^*$, given by a similarity score,
\begin{align*}
    \mathit{score}(x,e) = \text{cos}(M(x), M(e)).
\end{align*}
We experiment with RoBERTa~\cite{liu2019roberta} and SBERT~\cite{reimers2019sentence} as embedding models. We also try BM25~\cite{robertson2009probabilistic}, a retriever based on surface text similarity. We find SBERT leads to the best result; therefore, all IC-DST results reported here 
use SBERT as the retriever.

\paragraph{Retriever finetuning}
We also finetune SBERT on the few-shot examples to get a retriever that is better matched to the objective of predicting state changes. We first define the similarity between state changes. Suppose there are two sets of state changes, $c_a=\{(s_1^a, v_1^a), \cdots, (s_m^a, v_m^a)\}$, $c_b=\{(s_1^b, v_1^b), \cdots, (s_n^b, v_n^b)\}$. 
Let $F(set_1, set_2)$ be the average of two $F_1$ scores calculated by using $set_1$ vs. $set_2$ as the target.
Here we use the standard definition $F_1=\frac{2PR}{P+R}$, in which $P$ is precision, and $R$ is recall.
We define the slot similarity as
\begin{align*}
    F_{\mathit{slot}} = F(\{s_1^a, \cdots,s_m^a\}, \{s_1^b, \cdots, s_n^b\}) ,
\end{align*}
and the slot-value pair similarity as
\begin{align*}
    F_{\mathit{slot\mbox{-}value}} = F(&\{(s_1^a, v_1^a), \cdots,(s_m^a, v_m^a)\},\\
    &\{(s_1^b, v_1^b), \cdots, (s_n^b, v_n^b)\}) .
\end{align*}
Then the similarity between $c_a$ and $c_b$ is
\begin{align*}
    s(c_a, c_b) = \frac{1}{2}(F_{\mathit{slot}} + F_{\mathit{slot\mbox{-}value}}) .
\end{align*}
% \mocomment{It is not obvious what it means to "respect both...". You need to more concretely define this.} 

The positive and negative examples for training sample $x_i = (e_i, c_i)$ are identified by computing $s(c_i, c_j)$ for each sample $x_j=(e_j, c_j)$, sorting, and taking the $k$ highest  and lowest scoring samples, respectively.
We finetune the embedding model $M$ with a contrastive loss so that the similarity between a positive example pair is high and the similarity between a negative example pair is low.



% \subsection{In-Context Tuning}



% \begin{table*}[t!]
%     \small
%     \centering

%     \vspace{-0.5\baselineskip}
%     \begin{tabular}{lp{12.0cm}}
%         %\hline
%         \toprule
%         \textbf{Dialogue History} & [usr] i am looking for a italian restaurant centre . [sys] there are 9 restaurant -s that fit your request . what is your price range ? [usr] price does not really matter , but can you tell me the address , postcode , and phone for your favorite 1 ? [sys] my favorite is zizzi cambridge , located at 4753 regent street , cb21ab . their phone number is 01223365599 . would you like to reserve a table ? [usr] no thank you , but i am looking for a college to visit . [sys] any particular area ? [usr] no , it does not matter .  \\
%         \midrule
%         \textbf{\cite{hosseini2020simple}} &  attraction-area-dontcare, attraction-type-college, restaurant-area-centre, restaurant-food-italian, restaurant-pricerange-dontcare\\
%         \midrule
%         \textbf{SQL} (Ours) & \textbf{SELECT * FROM restaurant AS t1, attraction AS t2 WHERE t1.food = italian AND t1.pricerange = dontcare AND t1.area = centre AND t2.type = college AND t2.area = dontcare} \\
%         \bottomrule
%     \end{tabular}
%         \caption{An example pair of multi-domain dialogue state representations.}
%     \label{tab:example}
% \end{table*}

==> EMNLP 2022/sections/conclusions.tex <==
\section{Conclusion}
\vspace{-0.15in}

We successfully apply in-context learning for dialogue state tracking by introducing a new approach to representing dialogue context, a novel objective for retriever training, and by reformulating DST into a text-to-SQL task.
On MultiWOZ, our system achieves a new state of the art in both few-shot and zero-shot settings. 
Our analyses show that each innovation benefits performance.
We also study in detail the contribution of each design decision.
Future work may apply this in-context learning framework to a wider range of dialogue tasks.

%%MO: omit for blind review
\section{Acknowledgments}

This research was supported in part by funding from Allstate. We thank OpenAI for free access to Codex and Amazon for AWS credits.  %nascomment{did you use Amazon credits for this project?}




% \tao{to add an Acknowledgement section}

% \tao{cite the short semantic parsing paper on ARR: Evaluating the Text-to-SQL Capabilities of Large Language Models. Say about it in paper}


==> EMNLP 2022/sections/experiments.tex <==
\section{Experiments}
\label{experiments}


\input{tables/mw21}

\subsection{Datasets}
\label{datasets}

\paragraph{MultiWOZ~\cite{budzianowski2018multiwoz}} is a multi-domain human-human written dialogue dataset that contains over 10K dialogues across 8 domains.
The labels and utterances have been refined in subsequent versions, e.g., 
MultiWOZ 2.1~\cite{eric2019multiwoz}
and MultiWOZ 2.4~\cite{ye2021multiwoz}. MultiWOZ 2.4 is built on top of the 2.1 version and made substantial changes to the validation and testing sets. It can be viewed as a cleaner version of MultiWOZ 2.1 that better reflects model performance. In general, DST results are higher on 2.4 when compared to 2.1.\footnote{Many prior few-shot DST studies report results on MultiWOZ 2.1; we include this older version for direct comparisons.}
%  \nascomment{explain why we include 2.1?}\yushi{addressed in footnote.}
%\paragraph{DSTC 10~\michael{Don't have a paper to cite...}}
%Since Codex does not release the pretraining corpus, in order to prevent the model from accidentally memorizing the evaluation data, we choose to evaluate our systems on an additional corpus. The multi-domain dialogue state tracking task of DST10 track2 is chosen because it is released after Codex. In this task, new validation and testing set are collected in spoken form in order to test the robustness of task-oriented dialogue systems. %In both sets, only automatic transcriptions of dialogues are available. JGA is used as the main metric. 

% \paragraph{\yushi{New here}DSTC 10} track 2 is a challenge on knowledge-grounded spoken conversations. Here we focus on task 1 (multi-domain dialogue state tracking). The task provides development test sets with ASR outputs, and the participants are allowed to use any public data for training. We test our method on this task to address the potential test set leakage issue. This task is released later than Codex, and it is not included in Codex's training data.


\subsection{Baselines}
\label{baselines}

% \yushi{For truncation, skip this part}

\paragraph{TRADE~\cite{WuTradeDST2019}  }
An encoder-decoder framework is applied to the DST problem, enabling generalization to unseen values and domains. This was the first work to explore cross-domain transfer in DST. Different from IC-DST, TRADE has to make a prediction for each domain and slot pair in separate passes.

%\paragraph{SOLOIST~\cite{peng2020soloist}}
%Similar to ours, SOLOIST adopts an auto-regressive language model (i.e. GPT2). Dialogue states are generated conditioned on the whole dialogue history. But they are using direct finetuning, not in-context learning.  

%\paragraph{PPTOD~\cite{su2021multi}}
%In PPTOD, different task-oriented dialogue tasks (e.g. DST, intent recognition and reponse generation etc.) are used to pretrain a T5 model in a text-to-text format. 

\paragraph{SGP-DST~\cite{lee2021dialogue}}
In SGP-DST, schema information is used as a prompt to query a sequence-to-sequence language model (e.g., T5). It achieves SOTA on MultiWOZ 2.2. Similar to TRADE, the value for each domain and slot pair is predicted in a separate pass.

\paragraph{TransferQA~\cite{lin2021zero}}
TransferQA reformulated DST as QA problem. 
It is the state-of-the-art model for zero-shot DST.
The model is pretrained with a large amount of QA data. At inference time, the model predicts slot values by taking synthesized extractive questions as input.

\paragraph{DS2~\cite{shin2022dialogue}}
In DS2, DST is reformulated as a dialogue summarization problem. Sequence-to-sequence language models are trained with synthetic summary templates. The dialogue states can be recovered by reversing the template generation rules. This is by far the strongest few-shot model in the literature, outperforming recent few-shot models like T5-DST~\cite{lin2021leveraging}. However, different from us, this model still requires finetuning on DST labels.

% %\textbf{Few-Shot Learning} 
% %To demonstrate the few-shot learning abilities of our models, we randomly sample training set by 1\%, 5\% and 10\%, respectively. 
% %in ablation experiments, use MultiWoz 2.4. Use 5\% train data and 200 development dialogues.

% %\nascomment{the points about multiple passes make me think we should be measuring/reporting runtimes and potentially make claims about our method being faster.  worth considering?}\michael{Codex API has a call speed limit. It is hard to compare. One number I got from my SGPDST paper is 5.5x faster when using single pass.}

\subsection{Experimental settings}

% \mari{I moved some material from here to section 2, since I think that prompt examples and the zero-shot definition to be in the task definition section.}
%\yushi{new}
\paragraph{Few-shot setting} We follow the multi-domain scenario from ~\citet{wu2020improving}, where 1\%, 5\%, and 10\% of training data are sampled as the selection pool. The retriever is fine-tuned on the selection pool and does not see any other DST data. 
%%MO: I moved this to section 2
%A prompt example for this setting is given in Appendix~\ref{appendix:few shot}.
    
\paragraph{Zero-shot setting} 
\label{experiment_setting_zero_shot}
There are no labeled examples to retrieve, but a single formatting example turn is included, following previous zero-shot learning work~\cite{wang2022benchmarking}.
% \michael{I think it's better to be more transparent here about what the formatting examples are like. And don't have any annotated dialogues seems like a bit overclaim. Or I am being too critical?  : )}
% \yushi{I changed to only using one example so it's more "zero-shot". I also cited previous zero-shot work that has similar format}
%%MO: I moved this to section 2
%A prompt example for this setting is in Appendix~\ref{appendix:zero shot}.
%Here we assume that the system has the ontology for dialogue state tracking but does not have any annotated dialogues.
%Our prompt only contains a task instruction, which includes SQL tables as the dialogue schema, and, similar to previous zero-shot learning work~\cite{wang2022benchmarking}, one formatting example turn.  
%We call this setting ``zero shot'' because the prompt is fixed by the researchers and does not use any labeled data.
%\nascomment{I think we should be even more direct:  \emph{We call this setting ``zero shot'' because the prompt is fixed by the researchers and does not use any labeled data.} (not sure that's exactly right but you get the idea)}\yushi{Agree, copied in the text.}

\subsection{Experimental Details}

\paragraph{Language models}
\textbf{GPT3}~\cite{brown-gpt3} is a language model with 175B parameters pretrained on a large web corpus. It demonstrates strong zero-shot results on language modeling benchmarks.
Its successor, \textbf{Codex}~\cite{chen2021evaluating}, is pretrained using open-source code from Github.\footnote{\url{https://openai.com/blog/openai-codex/}}
This enables interesting applications such as code completion. 
In our initial studies, as in \cite{Shin2021FewShotSP}, Codex substantially outperforms GPT3; therefore, we use Codex for the following experiments.
In this paper, we use \textbf{Codex-Davinci}.\footnote{In particular, we use code-davinci-002 engine. 
Some papers mention that the model size of Codex-Davinci is 175B, but OpenAI does not officially confirm that.
}
In addition, we report results using \textbf{GPT-Neo} (2.7B) ~\cite{gpt-neo} and \textbf{CodeGen} (2.7B) ~\cite{Nijkamp2022ACP}. They are both pretrained on Pile~\cite{gao2020pile} and open-source code.


% \textbf{GPT-Neo}~\cite{gpt-neo} and 


% is a LM pretrained on Pile~\cite{gao2020pile}, an 825 GB English text corpus that is composed of 22 diverse datasets. 
% \textbf{CodeGen}~\cite{Nijkamp2022ACP} is a LM pretrained on Pile and open-source code.
% %In our experiments  we use \textbf{GPT-Neo} (2.7B) and \textbf{CodeGen} (2.7B). 


\paragraph{Evaluation}
The standard joint goal accuracy (JGA) is used as the evaluation metric.
It treats a prediction as correct only if for every domain all slots exactly match the ground-truth values. To be consistent with prior work~\cite{WuTradeDST2019}, we report all-domain JGA on few-shot settings and per-domain JGA on zero-shot settings. We also report the $F_1$ on slot-value pairs for analysis.



%\michael{TODO: bs, lr, epochs, deepspeed spec.}
%\yushi{TODO: Retriever training details}
%
\paragraph{\NAME details}
The retriever is initialized with SBERT all-mpnet-v2 (220M). We use AdamW optimizer~\cite{loshchilov2017decoupled} and set $2 \times 10^{-5}$ as learning rate, 1000 as warmup steps.
During retriever finetuning, for each training sample, we first compute similarity based on target labels. 
The positive and negative examples are the top and bottom 5\% samples among the 10\% nearest neighbors of the sample. 
This sampling strategy gives us hard negative examples.
The maximum length for retriever input is 512. 
With the dialogue state context representation, no turn contexts in MultiWOZ exceed this length limit.
For few-shot experiments,
we use 10 context exemplars in Codex experiments and 5 for GPT-Neo due to different length limits.
We set temperature to $0$ to enable greedy argmax sampling during generation.







==> EMNLP 2022/sections/introduction.tex <==


\begin{figure}[t]
  \includegraphics[width=0.49\textwidth]{fig/system-v3.pdf}
  \caption{
Illustration of DST task and \NAME approach. 
The task is to track the slot values associated with a user request up to the current turn (dialogue state). 
%%MO: shortened caption + I thought the superscript is confusable as footnotes
%Equivalently, we predict state change labels. 
%In this test turn, the user’s intention changes from booking a Catalan restaurant to booking a French restaurant. 
In few-shot settings,
given a test turn (1), \NAME first retrieves a few most similar turns from the labeled dialogues as examples (2). 
The task schema (not shown in the figure), examples, and the test dialogue turn are concatenated in the prompt to a LM (e.g. GPT3) (3) to produce the current turn dialogue state changes as a SQL query (4).
%In few-shot settings,
%given a test turn$^{(1)}$, \NAME first retrieves a few most similar turns from the labeled dialogues as examples$^{(2)}$. 
%The task schema (not shown in the figure), examples, and the test dialogue turn are concatenated in the prompt to a pretrained LM $^{(3)}$(e.g., GPT3 or Codex) to produce the current turn dialogue state changes as a SQL query$^{(4)}$.
}
  \vspace{-2mm}
  \label{fig:system}
\end{figure}


\section{Introduction}
\label{introduction}

%\mari{I moved the figure to section 2, where it is referenced}
% \begin{figure*}[t]
%     \centering
%     \includegraphics[width=0.8\linewidth]{fig/system.pdf}
%     \vspace{0.2in}
%     \caption{Illustration of our proposed in-context learning framework for dialogue state tracking. A dialogue retriever is first trained with the available \nascomment{this phrase `training data states label' does not scan for me.  unpack so it's more clear to a casual/rushed reader}  dialogue state changes labels of the training data (omitted in this diagram). In the inference stage, the testing dialogue is used as the query to retrieve dialogues with similar dialogue state changes. The prompt contains the SQL tables adapted from pre-defined schema, the retrieved dialogues, and the testing instance. A large LM (e.g., Codex) takes the prompt as input and decodes the predicted state changes. We represent dialogue states as SQL expressions to fully exploit Codex. For a full example of the prompt please refer to Appendix~\ref{appendix:prompt-example}.
%     \tao{to change}}
%     \label{fig:system}
% \end{figure*}

%\tao{paragraph 1: general intro to dialog state tracking. annotation cost/scalability? -> why few-shot is better.}

%\tao{paragraph 2: prior work in few-shot and their limitations. intro to in-context learning and its advantages and flexibility. even though it is widely used in other tasks, never on dialog DST yet.}

%\tao{paragraph 3: in this paper, we explore in-context learning for DST and achieve overall sota zero-shot/few-shot performance on mwoz and dstc 10. 
%1) first frame DST as text-to-SQL to better leverage Codex;
%2) retriever training methods overview;
%3) dialog context encoding methods.}


%\tao{paragraph 4: we study detailed analysis and show some interesting findings and conclusions:
%1) prompting formats;
%2) dialog retrieving methods;
%3) task formulation;
%4) others - improving acc on later turns, num of in context examples.}

% \input{tables/mw21}

%Task-oriented dialogue (TOD) systems have been widely used in real worlds for business like hotel reservation, food ordering, etc.
Dialogue state tracking (DST) is an important module in many task-oriented dialogue systems. 
The goal of this module is to extract users' intentions at each turn in the dialogue as represented in the slot values of a predefined schema. Collecting and annotating turn-level dialogue states is notoriously hard and expensive~\cite{budzianowski2018multiwoz}. Also, in commercial applications, it is common to extend the 
%%MO: rewrite to addres Tao's comment
schema and incorporate new domains. Thus, it is important to develop DST learning strategies that are flexible and scalable, in addition to requiring less data.
%DST systems to new domains and new schema. 
%Thus, it is important to develop DST systems in few-shot settings that rely on less annotated data. 
% \tao{rethink the logic: new domains/schema -> flexible and scalable dst systems}

%\yushi{changed to compare with zero-shot models}
%\mari{I did a major rewrite on this, since the flow was confusing to me and there were some cite problems}
Previous studies have explored zero/few-shot DST, but with some limitations.
%~\cite{wu2020improving,hosseini2020simple,lin2021leveraging, lin2021zero, li2021zero,su2021multi,Shin2022DialogueSA, lin2021leveraging,xie2022unifiedskg}.
%however, they have certain limitations. 
Most few-shot methods are based on finetuning pretrained language models \cite{wu2020improving, li2021zero,su2021multi,shin2022dialogue, lin2021leveraging,xie2022unifiedskg}. 
Such systems are less flexible, since they need to be retrained when new slots or domains are added, and finetuning large LMs is computationally expensive.
%To achieve good performance, for each new slot or domain added in the schema, or even new examples added, models need to be trained again, which is computationally expensive, and makes the system less flexible.
%Also, we need to retrain these systems again if we want to update the behavior of these systems after deployment.  
Most zero-shot methods have involved domain-transfer approaches \cite{hosseini2020simple,lin2021leveraging,lin2021zero}, which have not yielded good performance.
%, including multi-task training with related task-oriented domains \cite{hosseini2020simple,lin2021leveraging} and question-answering datasets \cite{lin2021zero}.
%Unfortunately, performance of these systems is quite low.
%Second, the zero-shot results are far from satisfying, and these methods often rely on labeled data from other tasks.
%or extra knowledge.
%For example, TransferQA~\cite{lin2021zero} relies on a large amount of QA data, 
%%MO: Lee et al. & Su et al. did not do zero-shot expts
%SGPDST~\cite{lee2021dialogue} leverages natural language descriptions of schemas, 
%and PPTOD~\cite{su2021multi} uses $\sim$2M dialogue utterances.


To address the above challenges, we propose the \NAME model to solve the DST problem with the in-context learning (ICL) paradigm~\cite{brown-gpt3}, in which a large language model makes predictions based on the task instruction and/or examples in the prompt.
In few-shot settings, the prompt contains exemplars that are retrieved from a small set of labeled training data. 
A motivation behind this framework is that it requires no finetuning (i.e., no parameter updates), which
makes systems
%in-context learning models 
flexible 
%and scalable 
in that they can handle queries in a new domain via the exemplar retrieval process \textit{without re-training}.
This enables developers to quickly prototype systems in new domains and rapidly leverage new collected data.
%%Move to 2.2
%Moreover, compared to traditional few-shot finetuning approaches, in-context learning allows control of the behavior of a system by simply updating in-context examples without re-training.
%%MO: You could add "or by retraining only the retriever"
%This approach has proven to be successful
ICL has been used successfully in semantic parsing ~\cite{Rajkumar2022EvaluatingTT,pasupat2021controllable,rubin2021learning}, especially in few-shot scenarios. 
However, these studies focus on sentence-level tasks. 
ICL has been explored for DST \cite{madotto2021few,xie2022unifiedskg}, but the performance fell short of pretraining and domain-transfer approaches to few/zero-shot learning. 
% DST introduces challenges for inference in the combination of a potentially long, two-party dialogue history with grounding in a structured ontology.
DST involves long, two-party dialogue histories with grounding in a structured ontology.
We believe these challenges cause the poor ICL performance on DST tasks in previous work.


%For instance, there is a length limit for LM prompting, so it is impossible to put as many dialogues as in-context examples in the prompt, compared with single sentences. 
%Also, retrieving dialogues as useful exemplars is difficult. 

%\mari{Revised to have highlight IC-DST formulation differences and connections to challenges, and to eliminate redundancy with bullets.}
To address these challenges, 
%of few/zero-shot learning for task-oriented dialogues, 
we explore in-context learning with three novel contributions. First, we reformulate DST as a text-to-SQL task, including a tabular description of the ontology in the prompt. This is a better match to the knowledge-grounded scenario, and it takes advantage of large language models pretrained with code:  Codex \citep{chen2021evaluating}, GPT-Neo~\citep{gpt-neo}, and CodeGen~\citep{Nijkamp2022ACP}. Second, we use the dialogue state in representing context, rather than the full conversation history, which is more efficient and better suited to domain changes. Lastly, in the few-shot scenario, we propose a new approach to learning a similarity score for selecting in-context examples that is trained to match similarity based on dialogue state changes. The \NAME approach, which incorporates these advances, achieves a new state of the art on MultiWOZ few-shot settings, i.e.\ when using 1--10\% training data. We also substantially improve the zero-shot state of the art by 10--30\% absolute accuracy on each domain.
A further contribution is an extensive analysis demonstrating impact from each innovation.


%To solve the length challenge of encoding long dialogue history, we rethink the dialogue representation in prompts. 
%We also propose an efficient way to learn a similarity score for dialogue contexts that is trained to match similarity based on dialogue state labels.
%This allows us to retrieve related exemplars that are more relevant to a particular test context. 
%The proposed dialogue retriever and the in-context learning framework can be applied to various kinds of dialogue tasks, not restricted to DST. 
%n addition, we propose to reformulate DST as a text-to-SQL task.
%This allows us to leverage the large language models pretrained with code:  Codex \citep{chen2021evaluating}, GPT-Neo~\citep{black2021GPT}, and CodeGen~\citep{Nijkamp2022ACP}.


%\nascomment{cut this paragraph; `extensive' is subjective and we don't want to overpromise.  instead, elaborate a bit in the bullet item I mark below}We also conduct extensive analyses to study what works and not for dialogue with in-context learning. Including but not limited to, how many training data is needed, what is the best unit for exemplar retrieval, what is the best output representation for dialogue states, and common errors of in-context learning. 
%In addition, we also explore reformulating DST into other tasks to better leverage the large language models.
%Dialogue states are used to interact with back-end databases to retrieve needed information via API calls. 

In summary, our work makes the following contributions:
\begin{itemize}

\item To our knowledge, we are the first to successfully apply in-context learning for DST, building on a text-to-SQL approach.
     
\item To extend in-context learning to dialogues, we introduce an efficient representation for the dialogue history and a new objective for dialogue retriever design.
     
\item Our system achieves a new state of the art on MultiWOZ in zero/few-shot settings.

\item We provide insights into how in-context learning works for dialogue, including the importance of good in-context examples and the LM's ability to generalize beyond examples.
%%MO: I don't think you need "but not limited to"
     
% \item We conduct extensive analyses to study what works and what doesn't work for dialogue with in-context learning, including but not limited to, the importance of dialogue retriever for in-context learning, what is the best unit for exemplar retrieval, what is the best output representation for dialogue states, and common error types for in-context learning approaches.

\end{itemize}


     %%MO: you don't have analyses where you expand the schema or domain, so I would not add anything on that in this version of the paper.
     %\tao{add more detail. also say: to demonstrate flexibility and scalability of IC-DST, we did...}%\nascomment{add a little detail here about what reader should actually expect}
     
     %\item We also provide detailed analyses of the key ingredients to successful in-context learning for dialogue, including retrieval unit selection, retriever training strategy and dialogue state representation selection.





% There are two paradigms of DST models, classification-based and generation-based models. A classification-based model assumes prior knowledge of all the possible values even for non-categorical slots. Whereas generation-based model decodes the value token-by-token and therefore possess the ability to generalize to unseen values. \\

% Generation-based DST models based on large pretrained language models achieve strong results without replying task-specific or domain-specific modules. Among them, auto-regressive models~\cite{hosseini2020simple} generate the states conditioned on the dialogue context via a uni-directional language model. Whereas, sequence-to-sequence models~\cite{lee2021dialogue} represent the dialogue context using a bi-directional encoder and generate the states via a separate decoder. Our work falls into the generation-based paradigm.\\

==> EMNLP 2022/sections/limitations.tex <==
\section{Limitations}
The performance of our framework is highly dependent on the inference language model, which may limit the framework's usage. 
For example, our framework may not work as well on speech recognition transcripts or other languages because of the lack of such data during language model pretraining.
Future work may explore the robustness and generalization ability of in-context learning, for which our \NAME can serve as a test bed.
% Also, every language model has an input length limit.
% Although we have made innovations in the dialogue representation to shorten input length, we may still run out of tokens in practice.
% For example, if the task contains a complex ontology, then the schema tables will take up the prompt space.
% Future work may explore smarter ways to incorporate the task schema and inputs into the prompt.
%Also, despite that \NAME does not require finetuning, we still need to do inference on large models like Codex to get good performance. 
Also, there is a tradeoff between avoiding the cost of fine tuning with a large language model vs.\ the cost of inference.
%Large language model inference leads to undesirable high energy usage and computational cost.
%%MO: I don't think you should mention the actual cost, since this could be different a month from now.
%For example, the cost of GPT3 inference is \$0.02 per 1k tokens.
Fortunately, thanks to the recent efforts in open-source large models like OPT~\cite{zhang2022opt} and BLOOM~\cite{BLOOM}, and model compression techniques like LLM.int8()~\cite{dettmers2022llmint8}, 
the cost of running large language models has been drastically reduced, and we are optimistic that this trend will continue in the future.
Further, it is possible to leverage zero/few-shot methods as a teacher model to generate “pseudo-labels” for training a system that has a lower inference cost, as in~\citet{ye2022zerogen}.
Future work may investigate more on low-cost approaches to applying in-context learning and large language models.

==> EMNLP 2022/sections/related_works.tex <==
\section{Related Work}

\paragraph{Dialogue state tracking}
Many DST systems have been proposed~\cite{WuTradeDST2019,zhang2020task,peng2020soloist,lin2020mintl,lee2021dialogue,zhao2022description,kim2020efficient,heck2020trippy}.
\citet{hosseini2020simple}, \citet{ham2020end} and \citet{peng2020soloist} use naive formats to represent the dialogue states. \citet{cheng2020conversational}, \citet{moradshahi2021contextual}, and \citet{platanios2021value} use hierarchical representations for dialogue states as in semantic parsing tasks.
To reduce the need for labeled data in DST, many approaches are proposed for few-shot DST~\cite{wu2020improving,li2021zero, gao2020machine, lin2021leveraging, campagna2020zero, su2021multi}. 
The state-of-the-art few-shot DST model is~\cite{shin2022dialogue}, in which the authors reformulate DST as a summarization task. We propose to represent the dialogue states as SQL and reformulate DST into a text-to-SQL task.

Most zero-shot methods have involved domain-transfer approaches, including multi-task training with related task-oriented domains \cite{hosseini2020simple,lin2021leveraging} and question-answering datasets \cite{lin2021zero}.
Unfortunately, performance of these systems is quite low.


\paragraph{In-context learning}
ICL of large PLMs like GPT3~\cite{brown-gpt3} has shown increasingly impressive few-shot performance on many NLP tasks.
ICL has obtained success in semantic parsing~\cite{pasupat2021controllable,rubin2021learning,Shin2021FewShotSP}, intent classification~\cite{yu2021few} and other primarily sentence-level tasks~\cite{min2021metaicl}.
To imitate ICL, \citet{pasupat2021controllable} finetuned a T5 model with inputs augmented by retrieved in-context examples.   
\citet{Shin2021FewShotSP} and \citet{Rajkumar2022EvaluatingTT} find that GPT3 or Codex can be generalized to produce different target programs with a few in-context exemplars.
%\tao{we need to cite this paper in the intro or prompting design part...}\yushi{has cited in intro}
\citet{xie2022unifiedskg} and \citet{madotto2021few} were the first to apply ICL for DST, but their systems underperform other methods.
Future work may consider improving dialogue retrieving methods and task prompting formulation.

\paragraph{Retrieval}
Most current work on ICL focuses on sentences or documents, while our task involves retrieving dialogues.
There are two general kinds of semantic retrievers.
The first is similarity-based retrieval. \citet{poesia2022synchromesh} and \citet{das-etal-2021-case} define a similarity metric between semantic parsing results and use this similarity as the training objective for the retriever. Another approach is LM-score based retrieval. \citet{rubin2021learning} and \citet{Shin2021ConstrainedLM} measure the quality of an example by the probability of a large language model decoding the correct answer. The $k$ highest and lowest quality samples are used as positive and negative samples for the retriever training. The most relevant retrieval studies on dialogue focus on tasks like knowledge identification~\cite{wu-etal-2021-dialki} and response selection~\cite{yuan2019multi, han2021fine}. Their tasks and settings are different from ours.

\vspace{-0.15in}

==> EMNLP 2022/sections/results.tex <==
\section{Results}
\label{result}

\input{tables/mw_zeroshot}

\paragraph{Few-shot DST on MultiWOZ}
Table~\ref{mw2.1results} shows the result on few-shot settings and full-shot settings of our \NAME compared with several recent baselines 
%discussed in Section~\ref{baselines} 
on MultiWOZ 2.1 and 2.4. 
As discussed in Section~\ref{datasets}, MultiWOZ 2.4 is a clean version of MultiWOZ 2.1 and therefore the performance is better. 
Our system achieves state-of-the-art performance for 1\%, 5\%, and 10\% few-shot learning settings using Codex, outperforming previous works that require model finetuning.  
When given more data as retrieval candidates, our systems improve.
%
GPT-Neo and Codegen have a similar trend but are generally worse than Codex and other baselines. This suggests that the size of language model matters when deploying ICL.

The prior ICL DST systems did not report on the standard few-shot configurations, so were not included as baselines.  However, our system represents a significant advance over these systems as well, substantially outperforming both UnifiedSKG~\cite{xie2022unifiedskg} (43.1\% vs.\ 23.5\% when using about 80 labeled dialogues) %\yushi{addressed Mari's comments here} 
and Few-Shot Bot~\cite{madotto2021few} (50.6\% vs.\ 13.9\%) on MultiWOZ 2.1.


\paragraph{Zero-shot DST on MultiWOZ}
% \michael{I think some folks are gonna challenge our definition of "zero-shot". Is there another way to present? For example, 5-shot?}
% \yushi{I changed to only using one crafted turn as demonstration example. It's not even a whole dialogue. As Noah suggested, in the experiment settings section I cited previous zero-shot work that also has demonstration examples.}
Table~\ref{mw_zeroshot} shows the zero-shot DST results on MultiWOZ 2.1 and 2.4. 
Our \NAME outperforms previous results by a large margin. 
In addition, \NAME has the advantage over these approaches that no training is required.
The multi-domain JGA of our \NAME is 35.3\% on MultiWOZ 2.4, which can be compared to 48.35\% for the system using few-shot learning with 1\% training (roughly 80 labeled dialogues).
%\yushi{Addressing Mari's comment on comparing with few-shot result: Notice that the evaluation metrics in Table~\ref{mw_zeroshot} is per-domain JGA. The multi-domain JGA of our \NAME is 30.5\% on MultiWOZ 2.4.}
SimpleTOD++~\cite{hosseini2020simple} and T5DST~\cite{lin2021leveraging} are
%The T5DST~\cite{lin2021leveraging} approach is 
trained on four domains on MultiWOZ and tested on the unseen domain. 
In addition, T5DST uses human-written slot descriptions to boost zero-shot performance.
TransferQA~\cite{lin2021zero} does not need any training on DST data.
However, each slot has to be reformatted into a question, and the model is trained on a large amount of QA data.
%%MO: no need to repeat this
%As mentioned in Section~\ref{experiment_setting_zero_shot}, we do not need a selection pool nor a retriever in this setting.
%For each test instance, the prompt only contains a fixed task instruction, consists of the SQL tables and one formatting example. The full prompt can be found in appendix~\ref{appendix:zero shot}.
%%MO: "The results" is ambiguous. Either say "our results" or "the results in Table 2"
Our results show the flexibility 
%and scalability 
of {\NAME}.
For each new domain or slot added, by updating the SQL tables and adding a demonstration example, the model attains good performance on the new ontology without any training.


% \input{tables/dstc10_zeroshot}

% \paragraph{Zero-shot DST on DSTC 10} 
% \michael{DSTC10 is not a popular benchmark and needs introduction. Our results on WOZ is already great. I prefer to remove DSTC10}
% \yushi{there are some problems. Some submissions have higher JGA, but they are trained with a lot of spoken language understanding data. Maybe we just do not include this dataset here to be free from trouble?}
% Table~\ref{dstc10} shows the zero-shot result on DSTC 10 track 2 task 1.
% Our \NAME achieves significantly higher JGA compared with the official TripPy~\cite{heck2020trippy} baseline, which is trained on MultiWOZ 2.1.
% Different from MultiWOZ, this task only provides ASR output. 
% The transcripts do not have punctuation, and the ASR errors hurt the performance.
% Nevertheless, our \NAME still get reasonable zero-shot performance.

==> EMNLP 2022/tables/errors.tex <==
\begin{table*}[th]
    \small
    \centering

    \vspace{-0.5\baselineskip}
    \begin{tabular}{l|p{13cm}}
        %\hline
        \toprule
        \textbf{Error type I} & \textbf{Noisy training example} \\
        \hline
        \textbf{Example} & [user] I need some information about churchill college.\\
        \textbf{Example label} & \textit{attraction-name: churchill college} \\
        \textbf{Test turn} & [user] I am hearing some good things about queens college, can you give me some basic info on them? \\
        \textbf{Prediction} & \textit{attraction-name: queens college} \\
        \textbf{Gold} & \textit{attraction-name: queens college, \textcolor{red}{attraction-type: college}} \\
        \midrule
        
        %\textbf{Error type} & \textbf{Missing named entities}\\
        %\hline
        %\textbf{Test turn} & [user] I am looking for city centre north bed and breakfast \\
        %\textbf{Prediction} & \textit{hotel-area: center, hotel-name: bed and breakfast} \\
        %\textbf{Gold} & \textcolor{red}{\textit{hotel-name: city centre north bed and breakfast}} \\
        %\midrule
        
        
        %\textbf{Error type} & \textbf{Missing information}\\
        %\hline
        %\textbf{Example} & [user] I need a place to stay please. A hotel would be great.\\
        %\textbf{Example label} & \textit{hotel-type: hotel} \\
        %\textbf{Test turn} & [user] Hotel would be better , can I get a phone number for 1 please? \\
        %\textbf{Prediction} & \textit{\{\}} \\
        %\textbf{Gold} & \textcolor{red}{\textit{hotel-type: hotel}} \\
        %\midrule
        %\textbf{Error type II} & \textbf{Confused by examples}\\
        %\hline
        %\textbf{Example} & [user] Yes, what moderate hotels are in the area?\\
        %\textbf{Example label} & \textit{hotel-pricerange: moderate}  \\
        %\textbf{Test turn} & [user] Are there any moderate 3 star hotels with free parking? \\
        %\textbf{Prediction} & \textit{hotel-pricerange: moderate} \\
        %\textbf{Gold} & \textit{hotel-pricerange: moderate, \textcolor{red}{hotel-stars: 3}} \\
        %\midrule
        
        %%MO: I changed the error names to all be noun phrases vs. a mix of grammatical types
         \textbf{Error type II} & \textbf{Retrieval limitations}\\
        \hline
        \textbf{Example} & [system] I found the Scudamores Punting co. and the Cambridge Punter. Which would you prefer? [user] I like the Cambridge Punter better. Can you give the phone number and postcode for them? \\
        \textbf{Example label} & \textit{attraction-name: Cambridge Punter}  \\
        \textbf{Test turn} & [system] There are 2 in the centre of town. Scudamores Punting co., and the Cambridge Punter. Would either of those interest you? [user] could you give me the address for the Cambridge Punter, please? I also need a place to stay , preferably somewhere cheap.\\
        \textbf{Prediction} & \textit{attraction-name: Cambridge Punter} \\
        \textbf{Gold} & \textit{attraction-name: Cambridge Punter, \textcolor{red}{hotel-pricerange: cheap}} \\
        \midrule
        
        
        \textbf{Error type III} & \textbf{Failure to generalize from examples}\\
        \hline
        \textbf{Example} & [user] I would like some information on places to stay in Cambridge. I prefer a guesthouse that includes free WiFi, parking does not matter. \\
        \textbf{Example label} & \textit{hotel-internet: yes, hotel-type: guest house, hotel-parking: don't care} \\
        \textbf{Test turn} & [system] What area of town would you like to be in? [user] It doesn't matter. I just want it to be a cheap guesthouse with WiFi included. \\
        \textbf{Prediction} & \textit{hotel-internet: yes, hotel-type: guest house} \\
        \textbf{Gold} & \textit{hotel-internet: yes, hotel-type: guest house, \textcolor{red}{hotel-pricerange: cheap, hotel-area: don't care}} \\
        \bottomrule
    \end{tabular}
        \caption{The most common error types of IC-DST Codex and their corresponding most similar examples. 
        %The errors are from dialogue PMUL4134, SNG01936, and MUL0088, respectively. 
        The missed slots in gold state changes are marked in red.}
    \label{tab:common error}
\end{table*}

==> EMNLP 2022/tables/formulation.tex <==
\begin{table}[h]\small
\centering

\begin{tabular}{lcc}
\toprule
& Traditional & Text-to-SQL \\
\hline
GPT-Neo 2.7B & 10.7 & 33.2 \\
CodeGen 2.7B & 17.6 & 30.6\\
Codex-Davinci & 49.1 & 58.7 \\
\bottomrule
\end{tabular}
\caption{
Comparison of DST generation target formulation using 5\% training data and Codex.
%\tao{Traditional format also uses CREATE TABLES?}}
The traditional format corresponds to the representation in SimpleTOD~\cite{hosseini2020simple}.
}
\label{formulation}
\vspace{-3mm}
\end{table} 


==> EMNLP 2022/tables/mw21.tex <==
\begin{table*}[th]
\small
\centering
% \begin{tabular}{P{1.7cm}P{1.2cm}P{1.2cm}P{1.0cm}P{1.2cm}P{1.2cm}P{1.2cm}P{1.1cm}P{1.1cm}P{1.1cm}}
\begin{tabular}{lrrrr|rrrr}
\toprule
& \multicolumn{4}{c}{MultiWOZ 2.1} & \multicolumn{4}{c}{MultiWOZ 2.4}\\
 Model & 1\% & 5\% & 10\% & 100\% & 1\% & 5\% & 10\% & 100\%\\
 \hline
 \multicolumn{9}{c}{Baselines (finetuned)} \\
 \hline
 TRADE~\cite{wu2020improving} & 12.58 & 31.17 & 36.18 & 46.00 & - & - & - & 55.05\\
 % TRADE + Self-supervision~\cite{wu2020improving} & 21.90 & 35.13  & 38.12  & - & - & - & - & -\\
% TOD-BERT~\cite{wu-etal-2020-tod} & 9.90 & 28.60 & 37.00 & 48.00 & - & - & - & - \\
 % SOLOIST\cite{peng2020soloist} (need run) & 36.4 & 37.1 & 37.9 & 56.85 \\
 SGPDST~\cite{lee2021dialogue} & 32.11 & 43.14 & 46.92 & 56.66 & - & - & - & - \\
 DS2 - BART~\cite{shin2022dialogue} & 28.25 & 37.71 & 40.29 & 46.86 & 30.55 & 42.53 & 41.73 & 46.14\\
 DS2 - T5~\cite{shin2022dialogue} & 33.76 & 44.20 & 45.38 & 52.32 & 36.76 & 49.89 & 51.05 & 57.85 \\
 \hline
 \multicolumn{9}{c}{In-Context Learning} \\
 \hline
 %Few-Shot Bot~\cite{madotto2021few} & -  &  -  & -  & 13.90 & - & - & - & -  \\
  %UnifiedSKG~\cite{xie2022unifiedskg} & -  &  -  & -  & 23.47 & - & - & - & - \\
  %\hline
 \NAME GPT-Neo 2.7B & 16.70  &  26.90  & 31.65  & 39.18 & 17.36  & 29.62 & 34.38  & 45.32 \\
 \NAME CodeGen 2.7B & 20.72 &  29.62  & 33.81  & 39.93 & 21.87  & 33.16 & 37.45  & 45.71 \\
 \NAME Codex-davinci & \textbf{43.13} & \textbf{47.08} & \textbf{48.67} & 50.65 & \textbf{48.35}  & \textbf{55.43}  & \textbf{56.88}  & 62.43\\
 %\multicolumn{4}{c}{In context tuning} \\
 %\hline
  %\NAME GPT-Neo & & 38.3 & ?? & 51.0 \\
 %GPT-Neo 2.7B & & &\\
\bottomrule
\end{tabular}
\caption{
\label{mw2.1results}
Multi-domain JGA evaluated on MultiWoz 2.1 and 2.4 using 1\%, 5\%, 10\%, and 100\% of the training set. 
The average results of 3 runs are reported. 
DS2-T5~\cite{shin2022dialogue} is the previous state-of-the-art few-shot DST model on MultiWOZ. 
%Note that Few-Shot Bot only experiments on the hotel domain. 
% \tao{1) consider to add more baseline results on mwoz 2.4. otherwise, followup papers would still prefer mwoz 2.1; 2) add a little detail explaining one of the baselines is a sota few-shot model (also some reviewers might wonder the few-shot performance of the model that achieves sota result in the full setting (e.g., Trippy 60\%?)).}
% \nascomment{explain what * and bold denote.  consider merging with the 2.4 table (just add four columns to the right?)}
}
% \bottomrule
 \vspace{-3mm}
\end{table*}

==> EMNLP 2022/tables/mw_zeroshot.tex <==
\begin{table*}[th]
\small
\centering
\begin{tabular}{lccccc}
\toprule
& attraction & hotel & restaurant & taxi & train\\
 \hline
 \multicolumn{6}{c}{MultiWOZ 2.1}\\
 \hline
SimpleTOD++~\cite{hosseini2020simple} & 28.01 & 17.69 & 15.57 & 59.22 & 27.75 \\
T5DST + description ~\cite{lin2021leveraging} & 33.09 & 21.21 & 21.65 & 64.62 & 35.42 \\
TransferQA ~\cite{lin2021zero} & 31.25 & 22.72 & 26.28 & 61.87 & 36.72 \\
\hline
 \NAME Codex & \textbf{59.97} & \textbf{46.69} & \textbf{57.28} & \textbf{71.35}  & \textbf{49.37}\\
 \hline
 \multicolumn{6}{c}{MultiWOZ 2.4}\\
 \hline
 \NAME Codex & \textbf{62.09} & \textbf{53.18} & \textbf{54.87} & \textbf{71.87}  & \textbf{51.42}\\
\bottomrule
\end{tabular}
\caption{
\label{mw_zeroshot}
Zero-shot per-domain JGA on MultiWOZ 2.1 and 2.4. 
%%MO: the JGA in the body is good enough.
For reference, the multi-domain JGA for IC-DST on MultiWOZ 2.4 is 35.3\%.
%%MO: I don't think you need this detail both in the caption and in the discussion.  I would move it to "baselines" actually.
%SimpleTOD++~\cite{hosseini2020simple} and T5DST~\cite{lin2021leveraging} are trained on four domains on MultiWOZ and tested on the unseen domain.
%TransferQA~\cite{lin2021zero} reformats DST as QA and is trained on QA tasks. 
%Our \NAME uses a fixed task instruction in the prompt.
}
\vspace{-3mm}
\end{table*}

==> EMNLP 2022/tables/prompting.tex <==
\begin{table}[h]\small
\centering

\begin{tabular}{lcr}
\toprule
Dialogue context & Example label & MW 2.4\\
representation &  (retrieval objective) & JGA \\
\midrule
full context & dialogue state &  45.0\\
prev.~state + single turn & dialogue state & 47.9\\
\hline
full context & state changes &  52.0\\
single turn & state changes & 55.8 \\
prev.~state + single turn & state changes & 58.7 \\
\bottomrule
\end{tabular}
\caption{
\label{prompting_method}
Comparison of DST dialogue context representation in prompt examples and different retrieval objectives, with 5\% of the training data and Codex. 
The retrieval objectives correspond to $F_1$ over all slot-value pairs in the dialogue state vs.\ just state changes.
%The dialogue context representations are illustrated in Figure~\ref{fig:representation}. 
%The example labels are exemplified in Figure~\ref{fig:state-changes}.
}
% \bottomrule
\vspace{-5mm}
\end{table}



==> EMNLP 2022/tables/retrievers.tex <==
\begin{table}[h]\small
\centering

\begin{tabular}{llcccc}
\toprule
&&\multicolumn{2}{c}{Copy} & \multicolumn{2}{c}{\NAME Codex} \\
&& JGA & $F_1$  &  JGA & $F_1$ \\
\hline
Unsuper. &Random & 0.7 & 4.9 & 29.8  & 81.1\\
 & BM25   & 4.9 & 31.8 & 49.0 &  91.0\\
 &SBERT  & 5.9 & 28.7 & 49.2 & 91.7\\
\hline
Super. & \textbf{Ours} & \textbf{16.3} & \textbf{61.4} & \textbf{58.7} & \textbf{93.3}\\
 \hline
 \hline
Oracle & $F_1$-oracle & 24.6 & 76.8 & 82.9  & 98.1\\
\bottomrule
\end{tabular}
\caption{
\label{retriever}
Comparison of different retrievers using 5\% of the training data and Codex. 
The ``copy'' baseline copies the label of  retrieved nearest example as prediction.
The oracle retriever assumes prior knowledge of the gold test instance dialogue state.
%%MO: I commented out details since it is in the analysis paragraph
%and retrieves examples with the highest state changes $F_1$.
%\nascomment{where is the oracle explained?} 
}
\vspace{-5mm}
\end{table}





==> sections/acknowledgements.tex <==
%\section*{Acknowledgments}
%We thank Ruiqi Zhong for generating test suite databases for our evaluation.
%%thank tianbao and chen too

==> tables/detail_numbers.tex <==
\begin{table*}[h]
\centering

\begin{tabular}{lcccccc}
\toprule
& \multicolumn{3}{c}{MultiWOZ 2.1} & \multicolumn{3}{c}{MultiWOZ 2.4} \\
& 1\% & 5\% & 10\%  & 1\% & 5\% & 10\% \\
\hline
 \multicolumn{7}{c}{GPT-Neo} \\
\hline
Run 1 & 18.44  & 26.24 &  32.10 & 19.29  & 28.79 &  35.22\\
Run 2 & 14.32  & 27.63 & 31.62 & 14.32  & 30.78 & 33.98\\
Run 3 & 17.35  & 26.83 & 31.23 & 18.46  & 29.30 & 33.93\\
\hline
Mean &  16.70 & 26.90 & 31.65 &  17.36 & 29.63 & 34.38\\
(Stdev) & (2.13) & (0.70) & (0.44) & (2.66) & (1.03) & (0.73)\\
\hline
 \multicolumn{7}{c}{CodeGen} \\
\hline
Run 1 & 22.11  & 29.33 &  33.70  & 23.25  & 33.03 &  37.83\\
Run 2 & 17.78  & 30.05 & 34.08 & 19.22  & 33.36 & 37.43\\
Run 3 & 22.27  & 29.47 & 33.66 & 23.13  & 33.08 & 37.08\\
\hline
Mean &  20.72 & 29.62 & 33.81 &  21.87 & 33.16 & 37.45 \\
(Stdev) & (2.55) & (0.38) & (0.23) & (2.29) & (0.18) & (0.38)\\
\hline
 \multicolumn{7}{c}{Codex} \\
\hline
Run 1 & 44.25  & 47.52 &  48.34 & 49.92  & 56.27 &  56.62\\
Run 2 & 41.99  & 47.18 & 49.04  & 47.31  & 54.33 & 56.65\\
Run 3 & 43.16  & 46.55 & 48.64 & 47.83  & 55.69 & 57.37\\
\hline
Mean &  43.13 & 47.08 & 48.67  &  48.35 & 55.43 & 56.88 \\
(Stdev) & (1.13) & (0.49) & (0.35) & (1.38) & (1.00) & (0.42)\\

\bottomrule
\end{tabular}
\caption{
Detailed test JGA in few-shot settings of MultiWOZ 2.1 and MultiWOZ 2.4.
}
\label{mw_details}
\vspace{-3mm}
\end{table*} 



